Linear Last-iterate Convergence in Constrained Saddle-point Optimization

Optimistic Gradient Descent Ascent (OGDA) and Optimistic Multiplicative Weights Update (OMWU) for saddle-point optimization have received growing attention due to their favorable last-iterate convergence. However, their behaviors for simple bilinear games over the probability simplex are still not fully understood - previous analysis lacks explicit convergence rates, only applies to an exponentially small learning rate, or requires additional assumptions such as the uniqueness of the optimal solution. In this work, we significantly expand the understanding of last-iterate convergence for OGDA and OMWU in the constrained setting. Specifically, for OMWU in bilinear games over the simplex, we show that when the equilibrium is unique, linear last-iterate convergence is achieved with a learning rate whose value is set to a universal constant, improving the result of (Daskalakis & Panageas, 2019b) under the same assumption. We then significantly extend the results to more general objectives and feasible sets for the projected OGDA algorithm, by introducing a sufficient condition under which OGDA exhibits concrete last-iterate convergence rates with a constant learning rate whose value only depends on the smoothness of the objective function. We show that bilinear games over any polytope satisfy this condition and OGDA converges exponentially fast even without the unique equilibrium assumption. Our condition also holds for strongly-convex-strongly-concave functions, recovering the result of (Hsieh et al., 2019). Finally, we provide experimental results to further support our theory.

==> experiments.tex <==
\section[Experiments]{Experiments} %\footnote{All source codes can be found at \url{https://github.com/bahh723/OGDA-last-iterate}.} %hide for submission 
\label{app:experiment}

\subsection{Matrix Games on Simplex}\label{app:a1}
Here we provide empirical results on the performance of \alg for matrix games on simplex. 
We set the size of the game matrix to be $32\times 32$, then generate a random matrix with each entry $G_{ij}$ drawn uniformly at random from $[-1,1]$, and finally rescale its operator norm to $1$.

We compare the performances of \alg and \OMWU. For both algorithms, we choose a series of different learning rates and compare their performances. We set $T=10^6$ and plot curves for $t=1,2,\dots,10^6$. 
\pref{fig:MGsimplex} shows the results. 
The $x$-axis of both plots represents time step $t$. 
The $y$-axis of the left plot represents $\ln(\KL(\z^\star, \z_t))$, the KL-divergence between $\z_t$ and $\z^\star$ after taking the natural logarithm. 
On the other hand, the $y$-axis of the right plot represents the logarithmic duality gap at each round $t$, which is 
\[
\ln (\alpha_f(\z_t))=\ln \left(\max_j( \G^\top \x_t)_j-\min_i(\G\y_t)_i\right).
\]
Note that here we use the limit point of $\z_t$ of \alg to be $\z^\star$. 
This is approximately calculated by running \alg much more than $T$ iterations (e.g. $10T$ iterations).
In fact, with probability $1$, the game has a unique Nash Equilibrium \citep{daskalakis2019last}. We also empirically verify that the iterates of \OMWU converge to the same point as \alg.
So the distance measure we use is reasonable.

From \pref{fig:MGsimplex}, we have the following observations. 
First, considering the convergence to Nash Equilibrium,  the curves of \alg with learning rate $\eta\in \{\frac{1}{8}, \frac{1}{4}, \frac{1}{2}\}$ are straight lines when $t> 2\times 10^5$, supporting the linear convergence of the distance shown in \pref{thm: point convergence}. 
The curves of \OMWU are also straight lines when $t$ is large. We tune a series of learning rates and the slope is quite small when $\eta$ is small. This also matches our theoretical results showing that \OMWU has a worse slope constant, which is exponentially small with respect to the least non zero value of the Nash Equilibrium. When $\eta$ grows, the slope also increases, though these values are not commonly used in practice, such as $\eta=5$ or $\eta = 10$.

Second, for the duality gap, the graph is roughly the same as the one for point-wise convergence. 
One minor difference for the plot of duality gap is that the curves for both algorithms are slightly oscillating, although they still converge linearly overall.

\subsection{Matrix Game on Curved Regions}
Next, we do experiments on a bilinear game similar to the one constructed in the proof of \pref{thm: bilinear-general}.
Specifically, the bilinear game is defined by \begin{align*}
f(\x,\y)={x_2}{y_1}-{x_1}{y_2},\quad\mathcal{X}=\mathcal{Y}\triangleq\{(a,b),0\le a,b\le 1,~a^n\le b\}.
\end{align*}
For any positive integer $n$, the equilibrium point of this game is $(0,0)$ for both $\x$ and $\y$.
Note that in \pref{thm: bilinear-general}, we prove that \alg only converges at a rate no better than $\Omega(1/t^2)$ in this game with $\mathcal{X}=\mathcal{Y}\triangleq\{(a,b),0\le a,b\le \frac{1}{2},~a^2\le b\}$.

\pref{fig:MGCurved} shows the empirical results for various values of $n$.
In this figure, we plot $\|\zp_t-\z^\star\|$ versus the time step $t$ in the log-log scale.
Note that in a log-log plot, a straight line with slope $s$ implies a convergence rate of order $\mathcal{O}(t^s)$, that is, a sublinear convergence rate.
It is clear from \pref{fig:MGCurved} that \alg indeed converges sublinearly for all $n$,
supporting our \pref{thm: bilinear-general}.


\begin{figure}
    \centering
	\includegraphics[width=0.49\textwidth]{A1-KL.pdf}
	\includegraphics[width=0.49\textwidth]{A1-Dual.pdf}\caption{Experiments of \alg and \OMWU with different learning rates on a matrix game $f(\x,\y)=\x^\top \G\y$, where we generate $\G\in \mathbb{R}^{32\times 32}$ with each entry $G_{ij}$ drawn uniformly at random from $[-1,1]$ and then rescale $\G$'s operator norm to $1$. The left graph shows the point-wise convergence results of \OMWU and \alg. The huge oscillation of \alg with $\eta=0.5$ is due to the numeric precision issue. The right graph shows the duality-gap convergence results of \OMWU and \alg. Both graphs show the linear convergence of \OMWU and \alg.}
	\label{fig:MGsimplex}
\end{figure}

\begin{figure}
    \centering
	\includegraphics[width=0.5\textwidth]{fig3.pdf}\caption{Experiments of \alg on matrix games with curved regions where $f(\x,\y)={x_2}{y_1}-{x_1}{y_2},\quad\mathcal{X}=\mathcal{Y}\triangleq\{(a,b),0\le a,b\le 1,~a^n\le b\}$, and $n=2,4,6,8$. This figure is a log-log plot of $\|\zp_t-\z^\star\|$ versus $t$, and it indicates sublinear convergence rates of \alg in all these games.} 
	\label{fig:MGCurved}
\end{figure}

\begin{figure}
    \centering
	\includegraphics[width=0.5\textwidth]{A3.pdf}\caption{Experiments on a strongly-convex-strongly-concave game where $f(\x,\y)={x_1}^2-{y_1}^2+2{x_1}{y_1},\mathcal{X}=\mathcal{Y}\triangleq\{(a,b),0\le a,b\le 1,~a+b=1\}$. The figure is a log graph of $\|\zp_t-\z^\star\|$ versus the time step $t$. The result shows that  \alg enjoys linear convergence and outperforms \OMWU in this case. }
	\label{fig:strongly}
\end{figure}

\subsection{Strongly-convex-strongly-concave Games}
In this section, we redo the experiments for strongly-convex-strongly-concave games in \citep{Lei2020Last}, where they consider the following case:
\begin{align*}
f(\x,\y)={x_1}^2-{y_1}^2+2{x_1}{y_1},\quad\mathcal{X}=\mathcal{Y}\triangleq\{(a,b),0\le a,b\le 1,~a+b=1\}.
\end{align*}
The equilibrium point is $(0,1)$ for both $\x$ and $\y$. In \pref{fig:strongly}, we present the log plot of $\|\zp_t-\z^\star\|$ versus time step $t$ and compare \alg with  \OMWU as in \pref{app:a1}. We also tune the learning rate respectively to make the comparison more reasonable.
The straight line curve of \alg implies that \alg algorithm converges linearly, supporting \pref{thm: strongly convex} and \pref{thm: point convergence}.
Also note that here, \alg outperforms \OMWU, which is different from the empirical results shown in \citep{Lei2020Last}.
We hypothesize that this is because they use a different version of \alg.

\subsection{An Example with $\beta > 0$ for \typetwo}
We also consider the toy example in \pref{thm: beta ge 0}, where 
$f(\x,\y)={x_1}^{2n}-{x_1}{y_1}-{y_1}^{2n}$ for some integer $ n \ge 2$
and $\mathcal{X}=\mathcal{Y}\triangleq\{(a,b),0\le a,b\le 1,~a+b=1\}$.
The equilibrium point is $(0,1)$ for both $\x$ and $\y$. We prove in \pref{thm: beta ge 0} that \typetwo does not hold for $\beta = 0$ but does hold for $\beta=2n-2$. 

The point-wise convergence result is shown in~\pref{fig:Nonstrongly}, which is again a log-log plot of $\|\zp_t-\z^\star\|$ versus time step $t$. One can observe that the convergence rate of \alg is sublinear, supporting our theory again. %Moreover, we can see that the slope of the curve for each $n$ is approximately $-\frac{1}{2n-2}=-\frac{1}{\beta}$, which means that $\|\hat{z}-z^\star\|\approxeq \Theta\left(t^{-\frac{1}{\beta}}\right)$. This result matches the upper bound shown in \pref{thm: point convergence}, showing that our theoretical result in~\pref{thm: point convergence} is tight in this case. 
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{fig5.pdf}\caption{Experiments of \alg on a set of games satisfying \typetwo with $\beta > 0$, where $f(\x,\y)={x_1}^{2n}-{x_1}{y_1}-{y_1}^{2n}$ for some integer $ n \ge 2$
and $\mathcal{X}=\mathcal{Y}\triangleq\{(a,b),0\le a,b\le 1,~a+b=1\}$. The result shows that \alg converges to the Nash equilibrium with sublinear rates in these instances. %Moreover, the slope of the curve is approximately $-\frac{1}{2n-2}$ for each $n$, matching the result shown in~\pref{thm: point convergence}.  
        }
        \label{fig:Nonstrongly}
\end{figure}

%\subsection{Stochastic Games}\label{app:a5}
%Finally, we show results for stochastic games. The algorithm we use is the original version of OGDA, that is, updating \pref{eq: sg update 2} and \pref{eq: sg update 4} with $Q^{s}_{t, t}$ instead of $Q^{s}_{t+1, t}$ and $Q^{s}_{t, t+1}$. 
%As discussed in \pref{sec:SG}, for the last-iterate convergence result, this does not matter.
 
%In the following we use $[K]$ to denote $\{1,2,\dots,K\}$ for some positive integer $K$.
%In this experiment, we set $H=4$, $\calA=\calB=[16]$, and $\calS_i=[8]$ for each $i\in [H]$ . 
%To expedite the convergence, we use $\eta=\frac{1}{8}$ instead of the learning rate suggested in \pref{thm:sg last iterate}.
%Both $\ell$ and $p$ are randomly generated.
%Specifically, each $\ell(s,a,b)$ is uniformly at random drawn from $[0,1]$.
%To generate $p(s'|s,a,b)$, we first choose $p'(s'|s,a,b)$ from $[0,1]$ uniformly at random,
%and then normalize it so that $p'(\cdot|s,a,b)$ is a distribution.
%\[
%p(s'|s,a,b)=\frac{p'(s'|s,a,b)}{\sum_{s'}p'(s'|s,a,b)}.
%\]

%The results are shown in \pref{fig:StocAlgs}.
%Similar to \pref{app:a1}, we compare \alg with \MWU, \OMWU, and \GDA.
%Also, we show the convergence of the duality gap and the distance. 
%The duality gap is defined as
%\begin{align}\label{eq:stocalpha}
%\alpha(\zp_t)=\alpha(\xp_t,\yp_t)=\max_{y}\rho_{\xp_t,y}-\min_{x}\rho_{x,\yp_t},
%\end{align}
%where $\rho_{x,y} = \E_{s\sim p_0} V^s_{x, y}$ and $p_0$ is set to be the uniform distribution supported on $\calS_1$.
%On the other hand, the distance is defined as the sum of the distance between $\zp^s_t$ and $z^s_\star$  over all states, where $z^s_\star$ is calculated in a similar way as in \pref{app:a1}.
%The conclusion of the results is also similar to that in \pref{app:a1}, with \alg outperforming others and enjoying a linear rate.

%We also compare convergence rates of \alg for different layers. 
%The results are shown in \pref{fig:StocLayers}.
%Here $\alpha(\zp_t,h)$, the duality gap of layer $h$ is same as $\alpha(\zp_t)$ defined in \pref{eq:stocalpha} except for different $p_0$, where we set to be the uniform distribution supported on $\calS_h$.  
%Similarly, the distance is defined as the sum of the distances over all states in layer $h$.
%It is not hard to see that there is no significant difference between different layers when comparing their convergences rates.
%However, our bound for the convergence rates has exponential dependence on layers.
%It would be an interesting direction to removing this dependence.
%\begin{figure}
    %\centering
    %\includegraphics[width=0.49\textwidth]{fig6.pdf}
    %\includegraphics[width=0.49\textwidth]{fig7.pdf}
    %\caption{Experiments of \alg and other algorithms on stochastic games. We set $H=4$, $\calA=\calB=[16]$, and $\calS_i=[8]$ for each $i$. Each $\ell(s,a,b)$ is uniformly drawn from $[0,1]$ at random.
    %As for $p(s'|s,a,b)$, we first choose $p(s'|s,a,b)$ from $[0,1]$ uniformly at random, and normalize them to form probability distributions. The result of \alg is compared with \MWU, \OMWU, and \GDA. Both of the point-wise convergence (left) and the duality gap convergence (right) are presented. %See \pref{eq:stocalpha} for the definition of the duality gap where $p_0$ is set to be the uniform distribution supported on $\calS_1$.
    %}
%    \label{fig:StocAlgs}
%\end{figure}
%\begin{figure}
%    \centering
%    \includegraphics[width=0.49\textwidth]{fig8.pdf}
%    \includegraphics[width=0.49\textwidth]{fig9.pdf}
%    \caption{Experiments of convergence of \alg on stochastic games in different layers. We set $H=4$, $\calA=\calB=[16]$, and $\calS_i=[8]$ for each $i$. Each $\ell(s,a,b)$ is uniformly drawn from $[0,1]$ at random.
%        As for $p(s'|s,a,b)$, we first choose $p(s'|s,a,b)$ from $[0,1]$ uniformly at random, and then normalize them to form probability distributions. We compare the convergence rates of different layers in the figures. Both of the point-wise convergence (left) and the duality gap convergence (right) are presented. % See \pref{eq:stocalpha} for the definition of the duality gap, where $p_0$ is set to be the uniform distribution supported on $\calS_h$ for each $h$.
%        }
%        \label{fig:StocLayers}
%\end{figure}

